CNN-based Lidar Point Cloud De-Noising in Adverse Weather

Lidar sensors are frequently used in environment perception for autonomous vehicles and mobile robotics to complement camera, radar, and ultrasonic sensors. Adverse weather conditions are significantly impacting the performance of lidar-based scene understanding by causing undesired measurement points that in turn effect missing detections and false positives. In heavy rain or dense fog, water drops could be misinterpreted as objects in front of the vehicle which brings a mobile robot to a full stop. In this paper, we present the first CNN-based approach to understand and filter out such adverse weather effects in point cloud data. Using a large data set obtained in controlled weather environments, we demonstrate a significant performance improvement of our method over state-of-the-art involving geometric filtering. Data is available at https://github.com/rheinzler/PointCloudDeNoising.

==> csv/overall_results_table.tex <==
\begin{scriptsize}%
\setlength{\tabcolsep}{2pt}
\begin{tabular}{l|cccc|cccc|cccc|cc|cc|cc|cc}
\toprule
\multirow{3}{*}{Approach}&\multicolumn{12}{c|}{IoU in \%} & \multicolumn{6}{c|}{points de-noised on road data in $\%$}&RT$^{3)}$&P$^{4)}$\\&
\multicolumn{4}{c|}{Exp 1} &
\multicolumn{4}{c|}{Exp 2} & 
\multicolumn{4}{c|}{Exp 3} &
\multicolumn{2}{c|}{Exp 1} &
\multicolumn{2}{c|}{Exp 2} &
\multicolumn{2}{c|}{Exp 3} &in&in\\&
{Clear} & {Fog} & {Rain} & {Mean} & 
{Clear} & {Fog} & {Rain} & {Mean} & 
{Clear} & {Fog} & {Rain} & {Mean} &
{Clear} & {Rain} &
{Clear} & {Rain} &
{Clear} & {Rain} &
ms & Mio \\ \toprule
%-----------------------------------------------------------number of samples
Samples Chamber$^{1)}$& 
14,386&29,777&28,637&72,800&
14,386&29,777&28,637&72,800&
14,386&29,777&28,637&72,800&
$-$ & $-$ & $-$ & $-$ & $-$ & $-$ 
100.0	& $4\mathrm{e}^{-6}$	\\ 
%-----------------------------------------------------------number of samples
Samples Road$^{1), 2)}$& 
$-$	  & $-$  & $-$  & $-$  & 
31,078& $-$  & $-$  & $-$  & 
34,381&34,381&34,381&103,143&
$-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\ \midrule
%-----------------------------------------------------------DROR
\textit{DROR} \cite{Charron2018} & 
88.13 	& 6.94 	& 7.37 	& 34.15 & 
88.13 	& 6.94 	& 7.37 	& 34.15 & 
88.13 	& 6.94 	& 7.37 	& 34.15 & 
3.93 	& 4.32	& 
3.93 	& 4.32	&
3.93 	& 4.32	&
100.0	& $4\mathrm{e}^{-6}$	\\ 

\input{csv/fig_tf_summaries_resubmit_03/IoU_metrics_transpose_eval_paper.tex}
\\
\bottomrule
\multicolumn{6}{r}{$^{1)}$ the column \textit{Mean} states the total number the samples}&
\multicolumn{5}{r}{$^{2)}$ fog and rain are augmented samples}&
\multicolumn{5}{r}{$^{3)}$ runtime (GeForce GTX 1080 Ti)}&
\multicolumn{5}{r}{$^{4)}$ number of trainable parameters}
\end{tabular}\vspace{-0.75cm}
\end{scriptsize}%
%lspci -nn | grep '\[03'
%1a:00.0 VGA compatible controller [0300]: NVIDIA Corporation GP102 [GeForce GTX 1080 Ti] [10de:1b06] (rev a1)
%68:00.0 VGA compatible controller [0300]: NVIDIA Corporation GP102 [GeForce GTX 1080 Ti] [10de:1b06] (rev a1)

==> csv/resubmit_03/test_exp02_metrics_all.tex <==
%clear&fog&rain&mean
\textit{exp01-LiLaNet-ckp-20000}&%--------------------exp01-LiLaNet-ckp-20000
82.72&79.57&88.16&83.48
\\
\textit{exp01-RangeNet21-ckp-15000}&%--------------------exp01-RangeNet21-ckp-15000
83.13&77.22&83.85&81.40
\\
\textit{exp01-RangeNet21-v2-ckp-15000}&%--------------------exp01-RangeNet21-v2-ckp-15000
71.53&71.40&86.13&76.35
\\
\textit{exp01-RangeNet53-v2-ckp-20000}&%--------------------exp01-RangeNet53-v2-ckp-20000
74.73&77.32&91.22&81.09
\\
\textit{exp01-WeatherNet-ckp-85000}&%--------------------exp01-WeatherNet-ckp-85000
91.65&86.40&89.29&89.11
\\
\textit{exp01-WeatherNet-v2-ckp-15000}&%--------------------exp01-WeatherNet-v2-ckp-15000
82.42&78.02&86.01&82.15
\\
\textit{exp01-WeatherNet-v2-ckp-20000}&%--------------------exp01-WeatherNet-v2-ckp-20000
83.32&78.92&85.77&82.67
\\
\textit{exp01-WeatherNet-v3-ckp-10000}&%--------------------exp01-WeatherNet-v3-ckp-10000
80.87&77.55&85.07&81.16
\\
\textit{exp01-WeatherNet-v3-ckp-15000}&%--------------------exp01-WeatherNet-v3-ckp-15000
80.63&77.86&85.62&81.37
\\
\textit{exp02-LiLaNet-ckp-10000}&%--------------------exp02-LiLaNet-ckp-10000
91.60&84.96&88.62&88.39
\\
\textit{exp02-LiLaNet-v2-ckp-20000}&%--------------------exp02-LiLaNet-v2-ckp-20000
92.34&86.30&89.25&89.30
\\
\textit{exp02-RangeNet21-v2-ckp-25000}&%--------------------exp02-RangeNet21-v2-ckp-25000
83.60&76.92&85.24&81.92
\\
\textit{exp02-RangeNet21-v2-ckp-30000}&%--------------------exp02-RangeNet21-v2-ckp-30000
86.71&80.90&87.01&84.87
\\
\textit{exp02-RangeNet53-v2-ckp-40000}&%--------------------exp02-RangeNet53-v2-ckp-40000
85.94&83.92&93.61&87.83
\\
\textit{exp02-RangeNet53-v2-ckp-45000}&%--------------------exp02-RangeNet53-v2-ckp-45000
87.75&86.46&94.23&89.48
\\
\textit{exp02-WeatherNet-v2-ckp-10000}&%--------------------exp02-WeatherNet-v2-ckp-10000
90.89&85.15&88.84&88.29
\\
\textit{-LiLaNet-ckp-95000}&%---------------------LiLaNet-ckp-95000
\textcolor{maxcolor}{93.85}&88.74&90.82&\textbf{91.14}
\\
\textit{-RangeNet21-v2-ckp-20000}&%---------------------RangeNet21-v2-ckp-20000
85.10&79.94&85.35&83.46
\\
\textit{-RangeNet53-v2-ckp-45000}&%---------------------RangeNet53-v2-ckp-45000
86.50&87.19&\textbf{94.36}&89.35
\\
\textit{-RangeNet53-v2-ckp-90000}&%---------------------RangeNet53-v2-ckp-90000
89.09&\textcolor{maxcolor}{90.58}&\textcolor{maxcolor}{94.66}&\textcolor{maxcolor}{91.44}
\\
\textit{-WeatherNet-ckp-50000}&%---------------------WeatherNet-ckp-50000
\textbf{93.35}&\textbf{88.81}&90.92&91.03
\\
\textit{-WeatherNet-v2-6e4-ckp-75000}&%---------------------WeatherNet-v2-6e4-ckp-75000
90.71&84.54&88.16&87.80
\\
\textit{-WeatherNet-v2-ckp-50000}&%---------------------WeatherNet-v2-ckp-50000
92.87&86.16&88.42&89.15
\\\bottomrule

==> img/boxplot_template.tex <==

\pgfplotsset{
    xticklabels from column names/.code={
        \pgfplotstableread{#1}\loadedtable
        \def\columnnamelist{}
        \pgfplotstableforeachcolumn\loadedtable\as\col{%
            \edef\columnnamelist{\columnnamelist\col,}
        }
        \pgfplotsset{xticklabels/.expand once=\columnnamelist}
    }
}

\newcommand{\MyBoxplot}{%
 boxplot/draw direction=y,
    ylabel={no of points},
    grid =both,
    %ytick = {0,15,30,45,60},
    xtick={0,1,2,3,4,5,6,7,8,9,10},
    xmin=0.5,xmax=10.5,
    boxplot/every box/.style={solid,fill=boxplot_fill, draw=boxplot_frame},
    boxplot/every whisker/.style={solid,draw=boxplot_whisker},
    boxplot/every median/.style={solid,draw=boxplot_median},
    boxplot/every outlier/.style={solid,draw=boxplot_outlier},
    style={thick}
    }
    
\newcommand{\DefineBoxplot}[2]{%
\newcommand{\aPlot}{img/lidar_static_objects/#1_no_points.csv}%
\newcommand{\bPlot}{img/lidar_static_objects/#1_mean_intensity.csv}%
\newcommand{\Mytitle}{#2}%


\pgfplotstableread[col sep = comma]{\aPlot}\mydata
\pgfplotstableread[col sep = comma]{\bPlot}\mydataB


\begin{tikzpicture}

\begin{groupplot}[group style={group size=1 by 2,horizontal sep=0.25cm, vertical sep=0.25cm}]
]
\nextgroupplot[%
    \MyBoxplot,
    title=\Mytitle,
    boxplot/draw direction=y,
    ylabel={no of points},
    xticklabels=none,
    xmajorticks=false
]%
        \foreach \i in {1,...,10} {
         %draw each originally row, now column as boxplot
            \addplot+ [mark=+,color=boxplot_outlier,  boxplot] table [y index=\i] {\mydata};
            }%
    \nextgroupplot[
    \MyBoxplot,
    ylabel={$\mathrm{mean}(i)$},
    xticklabels from column names=\bPlot,
    x tick label style={rotate=45},
    ]
        \foreach \i in {1,...,10} {
         %draw each originally row, now column as boxplot
            \addplot+ [mark=+,color=boxplot_outlier,  boxplot] table [y index=\i] {\mydataB};
            }%    
    \end{groupplot}
\end{tikzpicture}
}



==> img/cnn_network/encoder_decoder_block.tex <==
% -*- root: ../../root.tex -*-
%
% Define the layers to draw the diagram
\pgfdeclarelayer{network}
\pgfsetlayers{network,main}

\tikzstyle{nin}=[draw, fill=daiGreen4, text width=4.5em,text centered, minimum height=3.0em]
\tikzstyle{decoder}=[nin, fill=daiGreen4, trapezium, rotate=-90, trapezium left angle=70, trapezium right angle=70,  minimum height=2.0em, minimum width=0.5em, text width=0.5em]
\tikzstyle{encoder}=[decoder, rotate=180]
\tikzstyle{ende}=[draw, fill=daiGreen4, text width=4.0em,text centered, minimum height=2.5em]
\tikzstyle{wa} = [nin, text width=5.0em, fill=daiDeepRed7,minimum height=2.5em, rounded corners]

%draw,trapezium,trapezium left angle=70,trapezium right angle=0

% Define distances for bordering
\def\blockdist{1.3}
\def\edgedist{1.0}

\begin{tikzpicture}[trim left]
%------------------------------------------------------------------------
% ENCODER % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
%------------------------------------------------------------------------
%------------------------------------------------------------------------
% Input
%------------------------------------------------------------------------
\node (input) [wa] {Input\\Encoder};
%------------------------------------------------------------------------
% core
%------------------------------------------------------------------------
\node (encoder) at ([shift={(1.4*\blockdist,0)}]input.east)[nin]  {Conv $2 \times 2$};
\path [draw, ->] (input.east) -- node [above] {} (encoder.west);
\node[label={[rotate=45]right:\footnotesize n}] at ([shift={(-0.1*\blockdist,0.3*\blockdist)}]encoder.east) {};

\node (leaky) at ([shift={(1.1*\blockdist,0)}]encoder.east)[nin]  {Leaky Relu};
\path [draw, ->] (encoder.east) -- node [above] {} (leaky.west);
\node[label={[rotate=45]right:\footnotesize n}] at ([shift={(-0.1*\blockdist,0.3*\blockdist)}]leaky.east) {};

%------------------------------------------------------------------------
% output encoder
%------------------------------------------------------------------------
\node (output) at ([shift={(1.5*\blockdist,0)}]leaky.east)[wa] {Output\\Encoder};
\path [draw, ->] (leaky.east) -- node [above] {} (output.west);

%------------------------------------------------------------------------
% DECODER % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
%------------------------------------------------------------------------
%------------------------------------------------------------------------
% input 
%------------------------------------------------------------------------
\node (input1) at ([shift={(3.5*\blockdist,0)}]output.east)[wa] {Input\\Decoder};
%\path [draw, ->] (concat.east) -- node [above] {} (output.west);

%------------------------------------------------------------------------
% core decoder
%------------------------------------------------------------------------
\node (decoder) at ([shift={(1.4*\blockdist,0)}]input1.east)[nin]  {Transpose Conv $2 \times 2$};
\path [draw, ->] (input1.east) -- node [above] {} (decoder.west);
\node[label={[rotate=45]right:\footnotesize n}] at ([shift={(-0.1*\blockdist,0.3*\blockdist)}]decoder.east) {};

%------------------------------------------------------------------------
% Concat decoder
%------------------------------------------------------------------------
\node (concat1) at ([shift={(1.1*\blockdist,0)}]decoder.east) [nin]  {Concat};
\path [draw, ->] (decoder.east) -- node [above] {} (concat1.west);
%------------------------------------------------------------------------
% output decoder
%------------------------------------------------------------------------
\node (output1) at ([shift={(1.5*\blockdist,0)}]concat1.east)[wa] {Output\\Decoder};
\path [draw, ->] (concat1.east) -- node [above] {} (output1.west);

%------------------------------------------------------------------------
% Layout Encoder Block
%------------------------------------------------------------------------
\begin{pgfonlayer}{network}
\path[fill=daiCoolGrey,rounded corners, draw=black!50, dashed]
(encoder.west)+(-0.6*\edgedist,1.5*\edgedist) rectangle ([shift={(0.6*\edgedist,-1.5*\edgedist)}]leaky.east);
\end{pgfonlayer}
\path (encoder.south) +(-0.1*\blockdist,-0.5*\blockdist) node (encoderblock) {\large{\emph{Encoder Block}}};
\node[label={[rotate=45]right:\footnotesize n}] at ([shift={(-0.2*\blockdist,0.1*\blockdist)}]encoderblock.east) {};

%------------------------------------------------------------------------
% Layout Decoder Block
%------------------------------------------------------------------------
\begin{pgfonlayer}{network}
\path[fill=daiCoolGrey,rounded corners, draw=black!50, dashed]
(decoder.west)+(-0.6*\edgedist,1.5*\edgedist) rectangle ([shift={(0.6*\edgedist,-1.5*\edgedist)}]concat1.east);
\end{pgfonlayer}
\path (decoder.south) +(-0.1*\blockdist,-0.5*\blockdist) node (decoderblock) {\large{\emph{Decoder Block}}};
\node[label={[rotate=45]right:\footnotesize n}] at ([shift={(-0.2*\blockdist,0.1*\blockdist)}]decoderblock.east) {};

%
%\begin{pgfonlayer}{network}
%\path[fill=black!20,rounded corners, draw=black!50, dashed]
%(decoder.west)+(-0.6*\edgedist,1.0*\edgedist) rectangle ([shift={(0.6*\edgedist,-1.0*\edgedist)}]concat1.east);
%\end{pgfonlayer}
%\path (concat1.south) +(-0.1*\blockdist,-1.0*\blockdist) node (decoderblock) {\large{\emph{Decoder Block}}};
%\node[label={[rotate=45]right:\footnotesize n}] at ([shift={(-0.2*\blockdist,0.1*\blockdist)}]decoderblock.east) {};


%------------------------------------------------------------------------
% skip
%------------------------------------------------------------------------
\draw [draw, ->] (input.north)    -- +(0,.50)  -| (concat1.north);
%\draw [draw, ->] (decoder2.west)    -- +(0,.25)  -| (encoder2.east);

\end{tikzpicture}


==> img/cnn_network/lila_net.tex <==
% -*- root: ../../root.tex -*-
%
% Define the layers to draw the diagram
\pgfdeclarelayer{network}
\pgfsetlayers{network,main}

\tikzstyle{nin}=[draw, fill=blue!20, text width=4.5em,
text centered, minimum height=2.5em]
\tikzstyle{wa} = [nin, text width=5.0em, fill=green!20,
minimum height=2.5em, rounded corners]

% Define distances for bordering
\def\blockdist{1.3}
\def\edgedist{1.0}

\begin{tikzpicture}[trim left]

%------------------------------------------------------------------------
% Input
%------------------------------------------------------------------------

\node (distance_input) [wa] {Distance};
\path (distance_input.south) +(0.0*\blockdist,-0.3*\blockdist) node (ditance_image) {\includegraphics[width=2cm, height = 5mm]{images/cylindricDistCropped.png}};
\node (intensity_input) at ([shift={(0*\blockdist,-1.55*\blockdist)}]distance_input.south) [wa] {Reflectivity};
\path (intensity_input.north) +(0.0*\blockdist,0.3*\blockdist) node (intensity_image) {\includegraphics[width=2cm, height = 5mm]{images/cylindricIntCropped.png}};

%------------------------------------------------------------------------
% Concat
%------------------------------------------------------------------------

\node (concat) at ([shift={(2.1*\blockdist,-0.6*\blockdist)}]distance_input.south) [nin]  {Concat};
\path [draw, ->] (distance_input) -| node [above] {} (concat.north);
\path [draw, ->] (intensity_input) -| node [above] {} (concat.south);

%------------------------------------------------------------------------
% LiLaBlocks
%------------------------------------------------------------------------

\node (llb1) at ([shift={(0.9*\blockdist,0)}]concat.east)[nin]  {\emph{LiLaBlock}};
\path [draw, ->] (concat.east) -- node [above] {} (llb1.west);
\node[label={[rotate=45]right:\footnotesize96}] at ([shift={(-0.1*\blockdist,0.3*\blockdist)}]llb1.east) {};

\node (llb2) at ([shift={(0.9*\blockdist,0)}]llb1.east)[nin]  {\emph{LiLaBlock}};
\path [draw, ->] (llb1.east) -- node [above] {} (llb2.west);
\node[label={[rotate=45]right:\footnotesize128}] at ([shift={(-0.1*\blockdist,0.3*\blockdist)}]llb2.east) {};

\node (llb3) at ([shift={(0.9*\blockdist,0)}]llb2.east)[nin]  {\emph{LiLaBlock}};
\path [draw, ->] (llb2.east) -- node [above] {} (llb3.west);
\node[label={[rotate=45]right:\footnotesize256}] at ([shift={(-0.1*\blockdist,0.3*\blockdist)}]llb3.east) {};

\node (llb4) at ([shift={(0.9*\blockdist,0)}]llb3.east)[nin]  {\emph{LiLaBlock}};
\path [draw, ->] (llb3.east) -- node [above] {} (llb4.west);
\node[label={[rotate=45]right:\footnotesize256}] at ([shift={(-0.1*\blockdist,0.3*\blockdist)}]llb4.east) {};

\node (llb5) at ([shift={(0.9*\blockdist,0)}]llb4.east)[nin]  {\emph{LiLaBlock}};
\path [draw, ->] (llb4.east) -- node [above] {} (llb5.west);
\node[label={[rotate=45]right:\footnotesize128}] at ([shift={(-0.1*\blockdist,0.3*\blockdist)}]llb5.east) {};

\node (final) at ([shift={(0.9*\blockdist,0)}]llb5.east)[nin]  {Conv $1 \times 1$};
\path [draw, ->] (llb5.east) -- node [above] {} (final.west);
\node[label={[rotate=45]right:\footnotesize13}] at ([shift={(-0.1*\blockdist,0.3*\blockdist)}]final.east) {};

%------------------------------------------------------------------------
% output
%------------------------------------------------------------------------

\node (output) at ([shift={(1.5*\blockdist,0)}]final.east)[wa] {Semantic};
\path [draw, ->] (final.east) -- node [above] {} (output.west);

\path (output.north) +(0.0*\blockdist,0.3*\blockdist) node (output_image) {\includegraphics[width=2cm, height = 5mm]{images/semanticExampleSem.png}};

%------------------------------------------------------------------------
% Layout
%------------------------------------------------------------------------

\begin{pgfonlayer}{network}
\path[fill=black!20,rounded corners, draw=black!50, dashed]
(concat.west)+(-0.6*\edgedist,1.5*\edgedist) rectangle ([shift={(0.6*\edgedist,-1.5*\edgedist)}]final.east);
\end{pgfonlayer}

\path (final.south) +(-0.2*\blockdist,-0.45*\blockdist) node (lilanet) {\large{\emph{LiLaNet}}};

\end{tikzpicture}

==> img/daimler_color.tex <==
%daimer color schemes (http://styleguide.daimler.com/stilelemente/farben/)
%GRAY
\definecolor{daiCoolGrey} {RGB}{230,230,230}
\definecolor{daiCoolGrey1}{RGB}{68,68,68}
\definecolor{daiCoolGrey2}{RGB}{112,112,112}
\definecolor{daiCoolGrey3}{RGB}{158,158,158}
\definecolor{daiCoolGrey4}{RGB}{200,200,200}
%BLUE
\definecolor{daiPetrol} {RGB}{0,103,127}
\definecolor{daiPetrol1}{RGB}{0,51,60}
\definecolor{daiPetrol2}{RGB}{0,67,85}
\definecolor{daiPetrol3}{RGB}{0,86,106}
\definecolor{daiPetrol4}{RGB}{0,122,147}
\definecolor{daiPetrol5}{RGB}{80,151,171}
\definecolor{daiPetrol6}{RGB}{121,174,191}
\definecolor{daiPetrol7}{RGB}{166,202,216}
%RED
\definecolor{daiDeepRed} {RGB}{114,23,12}
\definecolor{daiDeepRed1}{RGB}{68,14,7}
\definecolor{daiDeepRed2}{RGB}{90,19,10}
\definecolor{daiDeepRed3}{RGB}{159,25,36}
\definecolor{daiDeepRed4}{RGB}{255,0,0}
\definecolor{daiDeepRed5}{RGB}{140,70,60}
\definecolor{daiDeepRed6}{RGB}{170,115,110}
\definecolor{daiDeepRed7}{RGB}{200,160,160}
\definecolor{daiDeepRed8}{RGB}{230,210,210}
% ORANGE
\definecolor{daiOrange} {RGB}{230,145,35}
\definecolor{daiOrange1}{RGB}{235,165,80}
\definecolor{daiOrange2}{RGB}{240,190,125}
\definecolor{daiOrange3}{RGB}{245,210,170}
\definecolor{daiOrange4}{RGB}{250,230,210}

% GREEN
\definecolor{daiGreen} {RGB}{110,160,70}
\definecolor{daiGreen1}{RGB}{140,180,110}
\definecolor{daiGreen2}{RGB}{170,200,145}
\definecolor{daiGreen3}{RGB}{200,200,180}
\definecolor{daiGreen4}{RGB}{225,235,220}

% define color bar
\definecolor{color0}{named}{daiPetrol}
\definecolor{color1}{named}{daiDeepRed}
\definecolor{color2}{named}{daiOrange}
\definecolor{color3}{named}{daiGreen}
\definecolor{color4}{named}{daiCoolGrey2}

% fog and rain color
\definecolor{colorFog}{RGB}{115,0,230}
\definecolor{colorRain}{RGB}{0,153,153}
\definecolor{colorClear}{RGB}{0,0,0}
\definecolor{colorValid}{named}{daiCoolGrey3}
\definecolor{colorInput}{named}{daiDeepRed3} %daiDeepRed
\definecolor{colorDenoised}{named}{daiGreen}
%define boxplot
\definecolor{boxplot_whisker}{named}{black}
\definecolor{boxplot_median}{named}{daiPetrol}
\definecolor{boxplot_frame}{named}{black}
\definecolor{boxplot_fill}{named}{white}
\definecolor{boxplot_outlier}{named}{daiDeepRed}

%\pgfplotsset{minor grid style={solid,line width=.1pt, daiCoolGrey3}}
%\pgfplotsset{major grid style={solid,line width=.1pt, daiCoolGrey3}}
%\pgfplotsset{outer axis line style={line width=0.1pt, daiCoolGrey2}}
%\pgfplotsset{height=4.305300000cm}
%\pgfplotsset{width=7.982465195cm}
%\usetikzlibrary{arrows,shapes,positioning}
%\usetikzlibrary{pgfplots.statistics}

==> img/datatool.tex <==
\DTLsetseparator{;}  
\DTLloaddb{databaseIoU3classDraft}{img/tensorboard/fig_tf_summaries_aggregate_to_fig_and_csv/IoU_metrics.csv}
\DTLloaddb{databaseIoU3class}{img/tensorboard/fig_tf_summaries_aggregate_to_fig_and_csv_dv13_3class_2class/IoU_metrics.csv}
\DTLloaddb{databaseIoU}{img/tensorboard/fig_tf_summaries_aggregate_to_fig_and_csv_dv13_3class_2class/IoU_metrics_transpose.csv}

%]\loadedtable{}

%\begin{tabular}{l
%		l
%		S[table-format = 3.0  ,round-precision=0]
%		S[table-format = 3.2  ,round-precision=2]
%		@{}l
%		
\newcount\rowidx

\newcommand{\columnthenrow}[2][0]{%
	\def\tabularcontents{\begin{tabular}{l
%				S[table-format = 2.2  ,round-precision=2]
				S[table-format = 2.2, table-omit-exponent, fixed-exponent = -2]
				S[table-format = 2.2, table-omit-exponent, fixed-exponent = -2]
				S[table-format = 2.2, table-omit-exponent, fixed-exponent = -2]
				S[table-format = 2.2, table-omit-exponent, fixed-exponent = -2]
							}\toprule &{Clear}&{Fog}&{Rain}&{mean IoU}}%
		\dtlforeachkey(\thiskey,\thiscol,\thistype,\thisheader)\in#2\do
		{%
			\ifnum\thiscol>#1\relax
			% header title
			\eappto\tabularcontents{%
				\noexpand\\\noexpand\midrule\expandonce\thisheader}%
			% row loop 
			\rowidx=0\relax
			\loop
			\advance\rowidx by 1\relax
			\DTLgetvalue{\thisvalue}{#2}{\rowidx}{\thiscol}%
			
			\eappto\tabularcontents{\noexpand&\expandonce\thisvalue}%
			\ifnum\rowidx<\DTLrowcount{#2}
			\repeat
			\fi
		}%
		\appto\tabularcontents{\\\bottomrule\end{tabular}}%
	\tabularcontents
}

\newcommand{\columnthenrowTwo}[2][0]{%
	\def\tabularcontents{\begin{tabular}{l
%				S[table-format = 2.2  ,round-precision=2]
				S[table-format = 2.2, table-omit-exponent, fixed-exponent = -2]
				S[table-format = 2.2, table-omit-exponent, fixed-exponent = -2]
				S[table-format = 2.2, table-omit-exponent, fixed-exponent = -2]
				S[table-format = 2.2, table-omit-exponent, fixed-exponent = -2]
							}\toprule &{Clear}&{Fog}&{Rain}&{mean IoU}}%
		\dtlforeachkey(\thiskey,\thiscol,\thistype,\thisheader)\in#2\do
		{%
			\ifnum\thiscol>#1\relax
			% header title
			\eappto\tabularcontents{%
				\noexpand\\\noexpand\midrule\expandonce\thisheader}%
			% row loop 
			\rowidx=0\relax
			\loop
			\advance\rowidx by 1\relax
			\DTLgetvalue{\thisvalue}{#2}{\rowidx}{\thiscol}%
			
			\eappto\tabularcontents{\noexpand&\expandonce\thisvalue}%
			\ifnum\rowidx<\DTLrowcount{#2}
			\repeat
			\fi
		}%
		\appto\tabularcontents{\\\bottomrule\end{tabular}}%
	\tabularcontents
}

==> img/fig_predict_results_denoising/denoise_results_resubmit_weathernet.tex <==
%------------------WeatherNet-------------------------------------------------------------------------------------------
%------------------pedestrian
\renewcommand{\pathtmpped}{./fig_predict_results_denoising/resubmission_02/exp03_WeatherNet/2018-11-26_153228_Dynamic-G2-Fog20_LidarImage_000000267} %
%------------------cyclist
\renewcommand{\pathtmpcyc}{./fig_predict_results_denoising/resubmission_02/exp03_WeatherNet/2018-11-26_153359_Dynamic-G4-Fog20_LidarImage_000000237}%

\subfloat[Raw Data]{\includegraphicstmp{%
\pathtmpcyc_gt.png}{Input}{\pathtmpped_gt.png}}
%
\subfloat[\textit{WeatherNet}]{\includegraphicstmp{%
\pathtmpcyc_prediction_noise_large.png}{Segmentation}{\pathtmpped_prediction_noise_large.png}}
%
\subfloat[\textit{De-Noised}]{\includegraphicstmp{%
\pathtmpcyc_denoised.png}{De-Noised}{\pathtmpped_denoised.png}}

%------------------RangeNet-------------------------------------------------------------------------------------------
%------------------pedestrian
\renewcommand{\pathtmpped}{./fig_predict_results_denoising/resubmission_02/exp03_RangeNet53/2018-11-26_153228_Dynamic-G2-Fog20_LidarImage_000000267} %
%------------------cyclist
\renewcommand{\pathtmpcyc}{./fig_predict_results_denoising/resubmission_02/exp03_RangeNet53/2018-11-26_153359_Dynamic-G4-Fog20_LidarImage_000000237}%

\subfloat[Raw Data]{\includegraphicstmp{%
\pathtmpcyc_gt.png}{Input}{\pathtmpped_gt.png}}
%
\subfloat[\textit{RangeNet53}]{\includegraphicstmp{%
\pathtmpcyc_prediction_noise_large.png}{Segmentation}{\pathtmpped_prediction_noise_large.png}}
%
\subfloat[\textit{De-Noised}]{\includegraphicstmp{%
\pathtmpcyc_denoised.png}{De-Noised}{\pathtmpped_denoised.png}}

==> img/fig_predict_results_denoising/denoise_results_road.tex <==
\renewcommand{\pathtmp}{./img/fig_predict_results_denoising/semseg_di_32_400_aug_both_sprinkles_full_LiLaBlockDil_1e3_2k5_ckp_40k_freeze/2018-01-17_143024_LidarImage_000000920}
\begin{figure*}
	\begin{tikzpicture}
		 \node[anchor=south west,inner sep=0, shift={(0,0)}] (image) at (0,0) {\includegraphics[width=0.49\linewidth,trim=7.0cm 1.750cm 4.00cm 2.0cm,clip]{\pathtmp_gt.png}};
		 \begin{scope}[x={(image.south east)},y={(image.north west)}]
		 				\node [anchor=north east] at (1.0150,1.040) {\includegraphics[width=0.175\linewidth,trim=1.0cm 0.00cm 7.5cm 0.0cm,clip]{./img/fig_predict_results_denoising/2018-01-17_143024_LidarImage_000000920_cam_frame_000001827.jpg}};	
		 \end{scope}
	\end{tikzpicture}
	\includegraphics[width=0.49\linewidth,trim=7.0cm 1.750cm 4.00cm 2.0cm,clip]{\pathtmp_prediction_noise_large.png}
	\caption{De-noising results shown on a snapshot with road data recorded during light rainfall. The result shows, that the
	approach is able to generalize the noise pattern and predicts valid results for real road recordings during
	rainfall. Note that the training and validation data set neither contains rain nor fog scenes on roads. The
	color coding is similar to Fig. \ref{fig:denoise_results_Dynamic-G2-Fog20}.}\vspace{-0.4cm}
	\label{fig:denoise_results_road_dense_rain}
\end{figure*}


==> img/plot_template.tex <==
\definecolor{myPurple}{named}{daiPetrol7}
\definecolor{myDarkPurple}{named}{daiPetrol}
\definecolor{myGreen}{named}{daiDeepRed8}
\definecolor{myDarkGreen}{named}{daiDeepRed}


\def\bottom#1#2{\hbox{\vbox to #1{\vfill\hbox{#2}}}}

\definecolor{tb_color_1}{RGB}{245,124,0}
\definecolor{tb_color_2}{RGB}{0,167,247}
  
%## cylce lists ####################################################################################
 \pgfplotscreateplotcyclelist{tb}{
 semithick,black\\%
 semithick,daiPetrol\\%
 semithick,daiDeepRed\\%
 semithick,daiGreen\\%
 semithick,daiOrange\\%
 semithick,dashed,black\\%
 semithick,dashed,daiPetrol\\%
 semithick,dashed,daiDeepRed\\%
 semithick,dashed,daiGreen\\%
 semithick,dashed,daiOrange\\% 
 }
 
\pgfplotscreateplotcyclelist{standard}{
%thick,solid,black\\%
thick,solid,daiPetrol\\%
thick,solid,daiDeepRed\\%
thick,solid,daiGreen\\%
thick,solid,daiOrange\\%
thick,solid,black\\%
thick,solid,daiPetrol\\%
thick,solid,daiDeepRed\\%
thick,solid,daiGreen\\%
thick,solid,daiOrange\\% 
}
\newcommand{\markerDefault}{mark options={thick, solid, scale=1}, mark repeat=4}

\pgfplotscreateplotcyclelist{mark}{
%thick,solid,black\\%
semithick,solid,daiPetrol,mark=square*, mark options={thick, solid, scale=0.8}, mark repeat=4\\%
semithick,solid,daiDeepRed, mark=*,mark options={thick, solid, scale=0.8}, mark repeat=4\\%
semithick,solid,daiGreen, mark=diamond*,mark options={thick, solid, scale=0.9}, mark repeat=4\\%
semithick,solid,daiOrange, mark=triangle*,mark options={thick, solid, scale=1}, mark repeat=4\\%
semithick,solid,black, mark=|,mark options={thick, solid, scale=1}, mark repeat=4\\%
semithick,solid,daiPetrol, mark=x,mark options={thick, solid, scale=1}, mark repeat=4\\%
semithick,solid,daiDeepRed, mark=oplus,mark options={thick, solid, scale=1}, mark repeat=4\\%
semithick,solid,daiGreen, mark=star,mark options={thick, solid, scale=1}, mark repeat=4\\%
semithick,solid,daiOrange, mark=otimes,mark options={thick, solid, scale=1}, mark repeat=4\\% 
}

 \definecolor{tb_color_1}{RGB}{245,124,0}
 \definecolor{tb_color_2}{RGB}{0,167,247}

 \pgfplotscreateplotcyclelist{tb}{
 semithick,black\\%
 semithick,daiPetrol\\%
 semithick,daiDeepRed\\%
 semithick,daiGreen\\%
 semithick,daiOrange\\%
 semithick,dashed,black\\%
 semithick,dashed,daiPetrol\\%
 semithick,dashed,daiDeepRed\\%
 semithick,dashed,daiGreen\\%
 semithick,dashed,daiOrange\\%
 }

%## defines for IEE 2 columns design ####################################################################################
\newdimen\mycm
\mycm=1cm
\newdimen\widthieeecolcm

\widthieeecolcm=8.636008694cm

%## default plot design ####################################################################################
\def\axisdefaultheight{3.75cm}
\pgfplotsset{compat=newest}
\pgfplotsset{table/search path={csv}, compat=1.15,
             ylabsh/.style={every axis y label/.style={at={(0,0.5)}, xshift=#1, rotate=90}}}
             
%minor ticks:
\pgfplotsset{minor grid style={thin, daiCoolGrey4}}
%major ticks: 
\pgfplotsset{major grid style={thin, daiCoolGrey4}}

%set grid
%\pgfplotsset{grid style={daiCoolGrey4}, grid=both}
\pgfplotsset{grid=both}
%\pgfplotsset{minor tick num=1}

%\def\axisdefaultheight{3.75cm}
%\widthieeecolcm=10.636008694cm

